Structure Preserving Stain Normalization of Histopathology Images Using Self-Supervised Semantic Guidance

Although generative adversarial network (GAN) based style transfer is state of the art in histopathology color-stain normalization, they do not explicitly integrate structural information of tissues. We propose a self-supervised approach to incorporate semantic guidance into a GAN based stain normalization framework and preserve detailed structural information. Our method does not require manual segmentation maps which is a significant advantage over existing methods. We integrate semantic information at different layers between a pre-trained semantic network and the stain color normalization network. The proposed scheme outperforms other color normalization methods leading to better classification and segmentation performance.

==> Misc.tex <==
% Color deconvolution methods first decompose light absorbing stain colors
% and then apply stain color components of the target image onto the input image.
% Ruifrok and Johnston [12] manually selected representative pixels to estimate the
% color deconvolution matrix. Rabinovich et al. [10] employed non-negative matrix
% factorization (NMF) to perform color deconvolution. However, this method can-
% not guarantee a global optimum since the problem is non-convex. Macenko et al.
% [9] used singular value decomposition (SVD) to achieve a closed-form solution.
% Vahadane et al. [14] added sparseness to restrict the solution space for NMF
% optimization. Besides, other methods were also proposed, such as blind color
% decomposition (BCD) [3] and stain color descriptor (SCD) [8].
%
%   Janowczyk et al. in \cite{Zhou19_6} sub-divide an input image into multiple tissue regions using a sparse autoencoder, and independently normalize each region. 
%


Wu et. al. in \cite{Gupta7} propose a generator-to-classifier network that jointly optimizes stain-translation and classification. 
%
%  Zanjani et al. \cite{Zanjani} use GANs with prior latent variables and an auxiliary network for stain normalization.
%
%
%In the case of template based methods, which is the case for most methods, the template may not be representative of the dataset leading to mismatch and poor performance.
%
% Zhou et. al. \cite{ZhouMiccai19} propose a color normalization GAN based on auxiliary inputs for color normalization of H\&E stained images.% We propose a stain normalization approach that uses segmentation information. %also propose an approach to automatically generate a stable stain color domain from the training set so that template is not needed.


% ------------------------
% , making it easier to get rid of the stain varia-
% tions thus improving the diagnosis process for both the pathologist and CAD
% systems. StainGAN is based on the . Cycle-consistency
% allows the images to be mapped to different color-model but preserves the same
% tissue structure. We evaluate our approach against the state of the art methods
% quantitatively and indirectly through a breast tumor classification. Our contribu-
% tions include 
% 2) Removing the need for a manually picked reference template, as our model
% learn the whole distribution. 3) Providing a benchmark for comprehensive com-
% parison between the proposed StainGAN method and most of the state of the
% art methods.

% ---------------------------------------------

% Our primary contribution is a color stain normalization method that uses segmentation information. We build our model using cyclic GANs \cite{cyclicGAN} as they are a popular and effective choice in previous approaches. As demonstrated in previous work \cite{prior,work} cycle GANs do a very good job of translating image appearances across different stain types, thus eliminaating the tedious task of selecting a reference stain. However, as pointed out by Gadermayr et. al. \cite{gadermayr2018} there is no guarantee that in the translated images shape integrity of underlying objects will be preserved. It is entirely possible that the shape outlines of translated objects changes. Consequently this leads to sub optimal performance especially when applied to segmentation tasks. 

% Change of shape outlines may not be critical for classification tasks since the decision is made on high level and low level features. However if a segmentation model is trained on the altered images and then used to segment new images it affects model performance. 

% Gadermayr in \cite{gadermayr2018} used a method with two separate pipelines for different tasks. Gupta et al.... in 
% gadermayr et al . in tmi ...........

% Our proposed approach makes use of segmentation information for color stain normalization. To overcome the pitfalls of altered structure shape in genrated images, Gadermayr \cite{gadermayr2018} used two different pipelines to alternate between translating images from one domain to domain. While their reported resutls are effective, the pipeline itself is tedious. Moreover in more recent work such as \cite{miccai2019papers} none have integrated segmentation information. 
% %
% We include segmentation information by generating information maps that highlight a fine grained segmentation of structures of the image. The information map not only highlights all structures but it also quantifies the relative importance of each pixel based on multiple features and scales. When this information is included in the loss function during training it ensures that the different structural information is preserved in the generated images.

% Refering back to Figure~\ref{fig:workflow} we depict that there is a ``information Map generation'' module that generates a weighted information of the image in a unsupervised manner. Since this does not require any prior annotations, the information map can be used during test time which significantly improves the performance of the color normalization. Training proceeds by integrating the segmentation loss into the cyclical   GAN framework and ensures that ..

% Below we describe each of the modules in greater detail



%For example, the information contained in depth features pertaining to the sky should not be used to generate depth features describing a pedestrian, and this behavior is now captured as a larger distance between their corresponding semantic features, which in turn produces smaller weights for that particular convolutional filter. 



% 4.2
% S EMANTIC G UIDANCE N ETWORK
% As the secondary network used to provide semantic guidance for the generation of depth features, we
% use a Feature Pyramid Network (FPN) with ResNet backbone (Lin et al., 2017). This architecture
% has been shown to be efficient for both semantic and instance-level predictions towards panoptic
% segmentation (Kirillov et al., 2019; Li et al., 2018; Xiong et al., 2019; Porzi et al., 2019). While
% our proposed semantically-guided architecture is not restricted to any particular network, we chose
% this particular implementation to facilitate the future exploration of different sources for guidance
% information. Architectural details follow the protocols described in Li et al. (2018), and unless
% mentioned otherwise the same pretrained model was used in all reported experiments. The semantic
% network is assumed fixed, pretrained on a held out dataset different than the raw data used for self-
% supervised learning, i.e. we do not require any semantic ground truth on the target dataset.

where $f_s$ is the feature map at multiple scales.% and the difference indicates pixel wise  

% V GG is the L2 distance between two images using all the multiple feature maps obtained from a pretrained V GG16 network [12]. This sums up to 64×2+128×
% 2+256×2+512×3+512×3 = 3968 feature maps and compares information from multiple scales for better robustness.
% All feature maps are normalized to values between [0, 1].

% As described previously in Section~\ref{sec:semguide} we process a given image through the pre-trained network to obtain output maps after each convolution stage. We calculate the difference in the feature maps of the two images (from domains $A$ and $B$) from their corresponding output stages. We term this loss as the feature map loss $L_{FeatMap}$ which is defined as :
% \begin{equation}
%     L_{FeatMap} = 
% \end{equation}

% Note that the different feature maps have varying sizes due to the multiple max pooling stages. Since the outputs of the corresponding stages have same dimensions we can take their pixel wise difference. $N_s$ denotes the size of the corresponding feature maps, and $n$ denotes the number of feature maps (corresponding to the number of filters) in that stage. The segmentation network also outputs a segmentation which we integrate into the training framework as the segmentation loss $L_{Seg}$ given by, 
% \begin{equation}
%     L_{Seg}= 
% \end{equation}

% \begin{equation}
%     L_{Seg} = {L_{FeatMap}(a,\hat{a}) + L_{FeatMap}(b,\hat{b})} + {L_{FeatMap}(a,a\hat{b}) + L_{FeatMap}(b,b\hat{a})}
%     \label{eq:segL}
% \end{equation}

% The framework consists of two generators, and two discriminators looking to distinguish between real and generated images. The transformed images from domain $A$ are expected to be similar to the images in domain $B$. This condition is captured in the adversarial loss. The cyclic loss ensures that the reverse mapping is also feasible. In addition to the above losses we propose to use a segmentation loss that captures the similarity between the segmentation maps generated by our self-supervised approach. 














%---------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

% Domain $A$ has images from multiple sources with various stain styles. To form domain $B$ with relatively uniform stain style, we follow \cite{ZhouMiccai19} to apply a k-means clustering technique on the stain color matrices of images in domain $A$ and retrieve a tight cluster as domain $B$. 


% In the original  cycle-GAN architecture, we translate images from
% domain A to domain B but not reversely since it is an n-to-1 mapping from
% domain A to domain B. In order to make the cycle-GAN work both ways, we
% use the stain color matrix as an auxiliary input to the network.

%  In forward cycle consistency, one
% image from domain $A$ (denoted as $a$) is translated to domain $B$ (denoted as $b̂$)  by generator $G_{AB}$ , expressed as b̂ = G A (a). Image b̂ is translated back to domain A (denoted as â), combined with pre-calculated stain color matrix W A of the original image and generator G B , i.e. â = G B ( b̂, W A ). Cycle consistency loss between a and â is calculated as 
% %
% \begin{equation}
%     L_{cycle} (Ga,Gb) = \E_{a∼p data (a)} \left[\left\|a − G B (G A (a), W A )\right\|_1 \right]
% \end{equation}

% In addition, discriminator DB is employed to distinguish between real image b
% and generated image b̂ where the adversarial loss in forward cycle L adv can be
% written as
% \begin{equation}
%     L adv (G A , D B , A, B) = E b∼p data (b) [log D B (b)]
% + E a∼p data (a) [log(1 − D B (G A (a)))].
% \end{equation}

% \subsubsection{Semantic Information from Segmentation Maps}

% Describe how the segmentation maps are used for training.
% Define $L_{seg}$ and present the full cost function.

% The backward consistency cycle behaves similarly as the forward cycle. Real
% image from domain B (denoted as b  ) is translated to domain A by genera-
% tor G B with corresponding stain color matrix W A calculated in Eq. 3. Output image â  is then used to generate b̂  by G A to calculate cycle consistency loss
% L cycle (G A , G B , B, W A ). Meanwhile, â  and real image a are used to train discrim-
% inator D A . Adversarial loss in backward cycle L adv (G B , D A , A, B) is calculated
% in a similar way as the forward cycle. The overall loss of our CNGAN expressed
% as
% L(G A , G B , D A , D B , W A ) = L adv (G A , D B , A, B) + L adv (G B , D A , A, B)
% + λ(L cycle (G A , G B , A, W A ) + L cycle (G A , G B , B, W A )).
% (6)
% The objective of our CNGAN is to maximize the loss in D A and D B and minimize
% the loss in G A and G B . The full objective of CNGAN is
% G ∗ A , G ∗ B = arg min
% max L(G A , G B , D A , D B , W A ).

% The architecture of generator G A is modified from Johnson et al. [7], which
% contains one stride-1 and two stride-2 convolutions and followed by nine residual
% blocks, two stride-2 transpose convolutions and one stride-1 convolution. Batch
% normalization is used between each layers. Network architecture of generator
% G B is the same as G A . The stain color matrix is tiled to the RGB channel of
% input image. For discriminators, 70 × 70 PatchGAN [5] is used: three stride-2
% and two stride-1 convolutions with leaky ReLU activation functions and batch
% normalization layers. Shrivastava et al.’s strategy [13] is used: 50 previously
% generated images are buffered and imported into discriminator instead of one
% latest generated image, which is effective to stabilize adversarial loss.



% The training procedure proceeds as follow: first, stain color matrix W A of
% input images from domain A is calculated and the forward cycle is run (a →

% b̂ → â). Next, the backward cycle is executed to translate real images b  from
% domain B to domain A and back to domain B (b  → â  → b̂  ) using the stain
% color matrix W A . Due to the guidance of W A , the translated color in both cycles
% are the same, which limits the diversity of color and thus reduces the oscillation
% of the loss function.
% After model is trained, the generator G A is capable of normalizing any stain
% color image to the color pattern in domain B.
% % ----------------------------------------------------



% forces the generator to maintain the image content without requiring paired
% samples. The identity-loss is applied to stabilize the training process as suggested
% in [9]. For training, standard data augmentation (rotation, flipping) is applied.
% Apart from a U-Net generator network [6], the standard configuration based
% on the patch-wise CNN discriminator is used [9] 1 . Initial learning rate is set to
% 0.0002. Adam optimizer is used.


% We evaluate the performance of our proposed color normalization method by using it as a preprocessing step for classification and segmentation of digital pathology images, and  examine whether it improves their performance. %We denote our method as $SegCN-Net$ (segmentation based color normalization network). Zhou et. al. in \cite{ZhouMiccai19} compared their stain normalization method's performance with  other approaches on multiple public datasets for disease classification. We follow a similar approach, using the same datasets and their results as baseline. Similar to \cite{ZhouMiccai19} the color normalization results  by Reinhard \cite{Zhou11}, Macenko \cite{Zhou19_9} and Vahadane et al. \cite{Vahadane} are also shown. 




% \subsection{Training and Implementation}

%A classifier trained and tested on images from the same center will give good performance.
%
%  Our second base line is a ResNet50 (ResNet$_{noNorm}$) with same settings as ResNet$_{1}$ trained on images of $C1_{16}$ and applied to images from $C1_{17} - C2_{17}$  without any colour normalization.  We again train a . The third baseline network is similar to ResNet$_{C17noNorm}$ except that $C1_{17} - C2_{17}$ images have been normalized before applying ResNet trained on $C1_{16}$ and denoted as ResNet$_{C17Norm}$%  with batch size $32$ and Adam optimizer learning rate of $0.001$ for $70$ epochs. This network without any stain normalization is denoted as $ResNet_{noNorm}$. 

% The primary aim of SegCN-Net is to investigate it's efficacy as a  preprocessing step and enable pre-trained classification or segmentation networks for use on new images from a different center.

% $SegCN-Net$ is to check whether the stain normalization can be used  our prposed 

% A successful stain normalization method should enable  a classification model trained on images of one center to be used for classification of images from another center. This is feasible since all the test images can be translated to domain $A$, the training domain. 
%Note that we have tried to replicate the results reported in \cite{ZhouMiccai19} to the best extent.
%Note that for all experiments the test set was the same. i.e., the test images from CAMELYON17 datset.  
%
%
% Of particular importance are the results of Vahadane et. al. \cite{Vahadane} and Zhou et. al. \cite{ZhouMiccai19}

%  \begin{figure}[h]
%  \centering
% \begin{tabular}{ccccc}
% \includegraphics[height=2.2cm, width=2.1cm]{Image1_r.jpg} & 
% \includegraphics[height=2.2cm, width=2.1cm]{Image2_r.jpg} & 
% \includegraphics[height=2.2cm, width=2.1cm]{Image21_Prop.jpg} & 
% \includegraphics[height=2.2cm, width=2.1cm]{Image21_Gader.jpg} & 
% \includegraphics[height=2.2cm, width=2.1cm]{Image21_Vahadane.jpg} \\
% (a) & (b) & (c) & (d) & (e) \\
% \end{tabular}
% \caption{Color normalization results: (a) Domain A image; (b) Domain B image;  Domain B transformed to Domain A using: (c) proposed $SegCN-Net$; (d) \cite{gadermayr2018miccai}; (e) \cite{Vahadane}. Areas of structure inconsistency are shown by yellow arrows.}
% \label{fig:segRes}
% \end{figure}

%  \begin{figure}[t]
%  \centering
% \begin{tabular}{ccccc}
% \includegraphics[height=2.3cm, width=2.3cm]{Image1_r.jpg} & 
% \includegraphics[height=2.3cm, width=2.3cm]{BlueImg2.jpeg} & 
% \includegraphics[height=2.3cm, width=2.3cm]{Img12_Our_Blue2.jpg} & 
% \includegraphics[height=2.4cm, width=2.3cm]{Img12_Gadermayr2.png} & 
% \includegraphics[height=2.4cm, width=2.3cm]{Img12_Vahadane2png.png} \\
% (a) & (b) & (c) & (d) & (e) \\
% \end{tabular}
% \caption{Color normalization results: (a) Domain A image; (b) Domain B image;  Domain A transformed to Domain B using: (c) proposed $SegCN-Net$; (d) \cite{gadermayr2018miccai}; (e) \cite{ZhouMiccai19}. Areas of structure inconsistency are shown by yellow arrows.}
% \label{fig:segRes}
% \end{figure}


% We trained the proposed model and a baseline CycleGAN model [8] for 20 epochs
% with ResNet-6 generator architectures and 70 × 70 PatchGANs discriminators.
% Hyperparameters are chosen similarly to [18] and we fix the embedding weight
% ω embd to be equal to the cycle consistency loss weight ω cyc (ω embd = ω cyc = 10).
% The training was distributed on 8 v100 GPUs using the Pytorch distributed
% computing library and the stochastic synchronous ADAM algorithm. We train
% the model on the Roche Pharma High Performance Computing (HPC) Cluster
% in Penzberg. The training lasted 9 h.



% \begin{table}[b]
%  \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline 
% %& \multicolumn{4}{|c|}{Comparison approaches} & Proposed \\ \hline
% {Method} & {Center$~1$}  & {Center$~2$}  & {Center$~3$} & {Center$~4$} & {Center$~5$} & {Average} & {$p$} \\  \hline
% {SegCN-Net$_{Seg~Only}$} & {0.9376} & {0.7974}  & {0.8942} & {0.9187} & {0.9012} & {0.8898}  & {0.0001} \\ \hline
% %
% {SegCN-Net$_{C17Rand}$} & {0.9624} & {0.8403}  & {0.9267} & {0.9478} & {0.9391} & {0.9232} & {0.34} \\ \hline
% {SegCN-Net$_{Glas}$} & {0.9762} & {0.8627}  & {0.9509} & {0.9677} & {0.9588} & {0.9432} & {0.042} \\ \hline
% \end{tabular}
% %
% \caption{AUC measures for Ablation studies on the CAMELYON17 dataset.}
% \label{tab:Ablation}
% \end{center}
% \end{table}


% Intuitively, using a pre-trained segmentation network for providing semantic information makes greater sense than using a pre-trained classification network. However, to quantify the relative contribution of each network we used a classification network with the following implementation details. We use the similar architecture as used for segmentation. However, instead of segmentation we train it to perform classification by replacing the final layer with a fully connected layer   ...... The network was trained on 
% We refer to this method as $proposed_{class}$. Corresponding to 

% \begin{table}[t]
%  \begin{center}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline 
% {} & \multicolumn{2}{|c|}{$SegCN-Net$}  & \multicolumn{2}{|c|}{Glas Rank 1}  & \multicolumn{2}{|c|}{\cite{gadermayr2018miccai}} & \multicolumn{2}{|c|}{\cite{ZhouMiccai19}} \\ \hline
% {} & {Part A} & {Part B} & {Part A} & {Part B} & {Part A} & {Part B} & {Part A} & {Part B} \\ \hline
% %
% {F1} & {\textbf{0.9351}} & {\textbf{0.7542}} & {0.912} & {0.716} & {0.926} & {0.728} & {0.922} & {0.729} \\ \hline
% {DM} & {\textbf{0.9212}} & {\textbf{0.8054}} & {0.897} & {0.781} & {0.909} & {0.798} & {0.892} & {0.785} \\ \hline
% {HD} & {\textbf{42.276}} & {\textbf{143.286}} & {45.418} & {160.347} & {44.243} & {157.643} & {\textbf{47.012}} & {\textbf{161.321}} \\ \hline
% \end{tabular}
% \caption{Segmentation results on the GLas Segmentation challenge for $SegCN-Net$, \cite{gadermayr2018miccai}, \cite{ZhouMiccai19} and the top ranked method. $HD$ is in mm. Best results per metric is shown in bold.}% HD is in mm}
% \label{tab:seg}
% \end{center}
% \end{table}
